Adversarial Robustness in Multi-Task Learning: Promises and Illusions

Vulnerability to adversarial attacks is a well-known weakness of Deep Neural networks. While most of the studies focus on single-task neural networks with computer vision datasets, very little research has considered complex multi-task models that are common in real applications. In this paper, we evaluate the design choices that impact the robustness of multi-task deep learning networks. We provide evidence that blindly adding auxiliary tasks, or weighing the tasks provides a false sense of robustness. Thereby, we tone down the claim made by previous research and study the different factors which may affect robustness. In particular, we show that the choice of the task to incorporate in the loss function are important factors that can be leveraged to yield more robust models.

==> LaTeX/4-rq1-old.tex <==
\section{RQ1: Adding Auxiliary Tasks}% VS single-task models}
\label{sec:rq1}

\subsection{Adversarial vulnerability against $l_\infty$ norm attacks and $l_2$ norm attacks}

\todored{Refactor section according to reviews}

Theoreom 3 showed that adversarial vulnerability decreases with the number of uncorrelated tasks. Its proof stems from the usage of the norm L2 with small perturbations and we would like to check if under this setting, increasing the number of tasks makes the model harder to attack.
%We evaluate in this context the impact of using norm L2 in our attacks, under low perturbation amount (epsilon=4), and limited attack steps (25).
%This configuration is the one demonstrated in Theorem 3 where multi-task learning improves the robustness of the models.
%makes it harder to attack individual and multiple tasks. %While improving the robustness against L2 attacks, multi-task learning provides little defense against L-infinite attacks. 

Figure~\ref{fig:impact-norm} covers 3 main tasks main tasks: semantic segmentation (s), z-depth (d) and normals (n). For each of the main tasks, the boxplot shows the range of relative task vulnerability of the multitask models we obtain by adding an other auxiliary task. We evaluate the relative task vulnerability against single-task and multi-task attacks with a limited perturbation budget ($\epsilon$=8/255, 25 attack steps). 

It confirms that adding auxiliary tasks helps improving the robustness of models against $l_2$ attacks. However, under $l_\infty$ attacks, the multi-task models remain vulnerable.% to adversarial attacks.
%the relative task vulnerability introduced by an L2 attack is very limited in comparison with what we can achieve with an L-infinite under the same configuration. %Additional figures about the other tasks are in Appendix C.


\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/norm/relative.png}}
\vskip -0.1in
\caption{Impact of attack norm on the relative task vulnerability of various tasks. Lower means more robust.}
\label{fig:impact-norm}
\end{center}
\vskip -0.2in
\end{figure}

%\subsection{Insights from figures in Appendix C.} 
\subsection{Robustness of Multi-task models under different settings}
In addition to the above experiments, we investigated the other factors which may affect the robustness of the models. This allows us to identify the key factors confirming or refuting the results of Theorem3. More precisely, we consider the perturbation budget $\epsilon$, the model architecture, and the number of training steps (the convergence of learning). We summarize our key findings below while detailed results are presented in Appendix C.

%Appendix C presents more figures on this section’s experiments. We evaluated the impact of multi-task learning under different settings and all showed that it provides limited robustness. They yield additional insights which we summarize here.

\paragraph{Attack budget $\epsilon$.} 
\label{epsilon_evaluation}
We evaluate the robustness of multitask models against attack size $\epsilon \in \{4/255,8/255,16/255,32/255\}$
Under strong adversarial attacks ($\epsilon > 4/255$), supplementary tasks do not provide reliable robustness both against single-task and multi-task adversarial attacks.

\paragraph{Model architecture.} 
\label{architecture_evaluation}
We evaluate the vulnerability of multi-task models on three families of encoders (Xception, Wide-Resnet, and Resnet) and for the latter, three sizes of encoders (Resnet18, Resnet50 and Resnet152).

Madry et al.\cite{madry2017towards} has shown on simple classification single-task datasets that smaller models are the most vulnerable against adversarial examples. 

Our results suggest that the contrary holds in the multi-task setting. Attacks on larger models cause more error under the same perturbation budget.

\paragraph{Training steps.} 
\label{steps_evaluation}
We evaluate different number of steps of the attack with steps $\in [1,50]$. Our experiments show that adding more training epochs improves both the clean performance and the robustness of models. \newline% against single-task and multi-task attacks.

\begin{mdframed}[style=MyFrame]
\textbf{
Answer to RQ1:}

\end{mdframed}

==> LaTeX/7_rq4-notable.tex <==
\section{RQ4: Task Selection}

Our previous results imply that one should carefully select the auxiliary tasks added to reduce model vulnerability. Generally speaking, the addition of auxiliary tasks can even have negative effects. Auxiliary task selection, however, comes with three drawbacks \cite{standley2020tasks}: the size of the model is bigger (due to the addition of the task-specific decoder), the convergence of the common encoder layers is slower, and the clean performance risk deteriorating as more tasks are added. This raises the question of how to select the combination that yields the lowest vulnerability \emph{without} evaluating the vulnerability of all the possible combinations. 

We propose three methods to make this selection more efficient. Their common idea is to compute a proxy of the adversarial vulnerability which is fast to get and correlated to the real adversarial vulnerability. 
%As before, we consider each possible pair of tasks with one main task and one auxiliary task. 
We use the relative task vulnerability of the models on the main task, as this metric is independent of the nature of the task (unlike 
%e.g., 
the task loss whose scale depends on the task). We use the Pearson coefficient to measure correlation as it captures the linear relationships between variables.

The first is early stopping, that is, training the model after a predefined (small) number of epochs. Here, we stop after 50 epochs while the full training lasts for 150 epochs. Strong correlations between the vulnerability of the models trained over these two number of epochs would indicate that one can decide which task combination is optimal after few 
%training 
epochs.

The second is to use a surrogate (less expensive) encoder and evaluate all task combinations on this encoder. We hypothesize that combinations of tasks that are effective when joint to the surrogate encoder are also effective with the original model. We validate this hypothesis by measuring the correlation between the vulnerability of the models formed by joining the surrogate encoder with any combination of tasks and the vulnerability of their counterparts using the original encoder. We use ResNet18 as the surrogate encoder and ResNet50 as the target encoder.

Our third selection method is guided by the clean performance that the model achieves on the main task when the auxiliary tasks are added. The existence of a correlation between clean performance and vulnerability would avoid the cost of evaluating adversarial vulnerability (e.g. applying PGD) and reuse existing results on clean performance predictions \cite{standley2020tasks} to 
%also 
predict adversarial vulnerability. 

We observe that all three proxy methods are correlated with the real adversarial vulnerability values. Specifically, early stopping offers a medium correlation (Pearson = 0.55, 4.23e-3) while the methods based on the surrogate encoder and the clean performance achieve a very strong correlation (Pearson = 0.94 / p-value=1.42e-12 and Pearson = 0.98 / p-value=1.91e-17 respectively).

\begin{mdframed}[style=MyFrame]
\textbf{
Answer to RQ4:} While exhaustively computing the adversarial vulnerability for all task combinations is computationally expensive, this cost can be significantly reduced with task selection%while obtaining a good approximation of the model vulnerability. 
In particular, guiding the auxiliary task selection by the clean performance or the vulnerability of a smaller surrogate %model 
offers reliable indications of the benefits achieved by adding these tasks.
%}
%\textbf{RQ4: We cannot infer the choice of the optimal combinations of tasks from their task transfer similarity, however evaluating their clean performances, their robustness in smaller models or after limited training can hint which combination of tasks are more robust.}
\end{mdframed}

%The fourth consists of  
%Our evaluation shows that auxiliary tasks that are comparatively better than others in mono-task attacks are also better in multi-task attacks (1) and that robust combinations of tasks in mono-task attacks are also robust combinations in multi-task attacks (2).

%In order to evaluate the relationships between tasks, we cannot immediately use the error or the loss values of the combinations as they have different scales and have different properties. Hence, we rely on the relative robustness metric we previously proposed and we use an ordinal approach to rank the interactions between the main task and each auxiliary as we assume that the task performance change monotonically. Starting from a matrix of relative task robustness (like Table~\ref{table:tasks-opt} A), we build a matrix of the pairwise tournament between the auxiliary tasks. For each row $k$ (main task), the column $i$ of the auxiliary task indicates the number of other auxiliary combinations of $k$ that have a lower relative robustness than the combination ($k$,$i$).
%where the auxiliary task $i$ provides a better performances. 

%We compare different settings and run the statistical tests in table~\ref{tbl:stats-atks}: 
%\emph{Pearson Correlation} on the relative task robustness metric and
%\emph{Kendall Tau ranking} on the ordinal rankings of auxiliary tasks.



%The link between robustness and task transfer is statistically negligible (3 and 4), contrary to the link between robustness and learning. It indicates that combinations of tasks that achieve higher clean performances are also the most robust (5 and 6).

%Next, we show that the robust combinations of tasks in one architecture are also robust in another architecture (8), and there is strong evidence (p-value = 0.002, effect size $>$ 0.5) that auxiliary tasks that support a task in one architecture also support this task on an other architecture (7).

%Similarly, we have that combination of tasks that are robust together with limited training remain the most robust with a larger training budget (11 and 12).

%Finally, we compared whether the overall robustness of the task combinations is similar between a Renet50 and a Resnet18 model, and according to the Wilcoxon Two-sided, we cannot reject the null hypothesis at a confidence level of 5\% that the two architectures provide similar performances. However, if we test the hypothesis that the robustness in a Resnet50 model is higher than the robustness in a smaller model, the Wilcoxon-test shows that this hypothesis can be rejected at a confidence level of 5\%. This confirms that having larger models does not statistically improve the robustness of a multi-task model.

% \begin{mdframed}[style=MyFrame]
% \textbf{RQ4: We cannot infer the choice of the optimal combinations of tasks from their task transfer similarity, however evaluating their clean performances, their robustness in smaller models or after limited training can hint which combination of tasks are more robust.}
% \end{mdframed}
%\textbf{We cannot infer the choice of the optimal combinations of tasks from their task transfer similarity, however evaluating their clean performances, evaluating their robustness in smaller models or after few training steps can also hint about which combination of tasks are preferable.}


%Knowing the robustness on two tasks (two by two), can we infer the robustness of 3 tasks? 

%The fact there is no correlation between transfer and robustness confirms that adding an auxillary task that is related to the main task according to Taxonomy (like D and d) does not make the model less or more robust.


%\paragraph{Collaborative tasks robustness}


%\subsection{Mono Robustness \& Multi-robustness}

%KendalltauResult(correlation=0.7240000000000001, pvalue=9.798288078869026e-06) 
%Pearson(0.8400000000000001, 1.5061643470464924e-07)

%\subsection{Robustness \& Transfer affinity}

%\paragraph{multi-task attacks:}
%Pearson Correlation between task robustness \& transfer affinity: (0.04063728734751635, 0.8470660239914007)
%Kendall Order correlation: KendalltauResult(correlation=0.12112702310050734, pvalue=0.44881922452403433)


%\paragraph{Mono-task attacks:}
%Pearson Correlation between task robustness \& transfer affinity: (0.11441169155894705, 0.5860528793676638)
%Kendall Order correlation: KendalltauResult(correlation=0.11721969977468451, pvalue=0.463586942852103)

%\subsection{Robustness on eps4 VS eps 8 VS eps16}

%\subsection{Robustness on epochs 5 VS 25 VS 50}

%\subsection{Noise per task}
%PSNR mean per task


%\subsection{Robustness \& Learning affinity}

%\subsection{Robustness \& Adversarial transferability}

==> LaTeX/_dense.tex <==
\section{Empirical evaluation}

%\begin{mdframed}[style=MyFrame]
%\begin{equation}
% f(x) = \sin(x)
%\end{equation}
%\end{mdframed}

\input{LaTeX/-hypothesis}
\input{LaTeX/-study_factors}

%\input{LaTeX/-study_attacks}

%------------------------------------------------------------------------
%\input{LaTeX/-study_architectures}

%------------------------------------------------------------------------
\input{LaTeX/-study_tasks}


==> LaTeX/_experimental_setup.tex <==
\section{Experimental setup}

%We focus our research on to families of tasks: Multi-task Classification using the UTK Face dataset \cite{zhifei2017cvpr} and the CNN model provided in its original paper, and Multi-task Dense Predictions using the Taskonomy dataset\cite{taskonomy2018} and various combinations of architectures. 

\subsection{Dataset}

%\paragraph{UTK Face dataset} is a large-scale face dataset of 20K images where we try to predict both the gender and the ethnicity. The images cover large variation in pose, facial expression, illumination, occlusion, resolution, etc. This dataset could be used on a variety of tasks, e.g., face detection, age estimation, age progression/regression, landmark localization, etc. 

%We focus on two classification tasks:
%\begin{itemize}
%    \item \emph{gender} (g) is either 0 (male) or 1 (female)
%    \item \emph{race} (r) is an integer from 0 to 4, denoting White, Black, Asian, Indian, and Others (like Hispanic, Latino, Middle Eastern).
%\end{itemize}


\paragraph{Taskonomy} dataset\cite{taskonomy2018} gathers 4.5M indoor scenes images. From the original paper, we focus on 11 tasks (semantic, 2D and 3D): Semantic Segmentation (s), Depth z-buffer Estimation (d), Depth euclidian Estimation (D), Surface Normal Prediction (n), SURF Key-point Detection in 2D (k) and 3D (K), Canny Edge Detection (e), Edge Occlusion (E), Principal Curvature (p), Reshading (r) and Auto-Encoders (A). We restrict our study on the "small" split of their dataset. 

We chose this dataset and not other popular dense task dataset because (1) it is one of the dataset with the most and diverse computer vision tasks; (2) it is regularly used in the literature to evaluate task similarity and transfer and (3) is provided with a taxonomy of tasks\cite{taskonomy2018} where similar tasks are grouped (in Figure~\ref{taskonomy-tree}.

Besides, previous work has shown that segmentation-focused datasets like Cityscape[] have less variability and are weak even against single-task attacks\cite{arnab2018robustness}. Hence, these datasets are not a suitable benchmark for our study.    

%In the main paper, we focus our visualisations and details on 5 tasks sorted according to the taxonomy proposed by Zamir et al.\cite{taskonomy2018} (that we show in Figure~\ref{taskonomy-tree}): D and d tasks are adjacent, E is farther in the tree leaves, then n and s is the farthest leave from d. Our aim was to cover a wide field of tasks then evaluate if this taxonomy has any impact on the robustness of the combined tasks.  

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/task_tree.jpg}}
\caption{Task similarity tree proposed by Zamir et al.\cite{taskonomy2018}. D and d tasks are adjacent, E is farther in the tree leaves, then n and s is the farthest leave from d. 
%Our aim was to cover a wide field of tasks then evaluate if this taxonomy has any impact on the robustness of the combined tasks.
We focus our figures on these 5 tasks to cover a diverse set of tasks.
}
\label{taskonomy-tree}
\end{center}
\vskip -0.2in
\end{figure}


\subsection{Attacks}

We focus our research on gradient-based attacks, in particular on the L-infinite Projected Gradient Descent attack \cite{pgd} with 25 steps attacks and an attack strength of $\epsilon=4$. We also evaluate other configurations of attacks in specific sections:

\begin{itemize}
    \item We evaluate different strength of attacks with PGD $\epsilon \in \{2,4,8,16\}$
    \item We evaluate different number of steps of the attack steps $\in [1,50]$ including the 1 step without random start that covers the FGSM attack.
    \item We compare the PGD attack with our two optimizations \textbf{MGD} and \textbf{MAGD}.
\end{itemize}

We provide in the supplementary materials the detailed configurations and results across all the tasks.

\subsection{Models}

%For the UTKFace dataset, We evaluate two models that have the same common trunk and share a different degree of head layers:
%\begin{itemize}
%    \item For M1: The task-specific branching only concerns the last dense layers, after the common features have been extracted for both tasks
%    \item for M2: The common tasks only concern the low-level features, while each task has its own high level features and dense layers. Which means that the tasks do no share the embedding features used for %classification.
%\end{itemize}
%Both tasks rely on a Cross-entropy loss. 

%We also evaluate two mono-tasks models, one for the gender task and one for the race task.

We use a standard encoder-decoder architecture. We evaluate 3 families of encoders (Xception, Wide-Resnet and Resnet) and for the later, evaluate three sizes of encoders (Resnet18, Resnet50 and Resnet152).
We use a Cross-entropy loss for the Semantic Segmentation task and a L1 loss for the other tasks.

For each architecture, we evaluated two settings of multi-task models. In the first one, we trained and evaluated the models on 2 tasks among the 11 with equal weights. In the second, we weighted the loss of each task according to the common practice\cite{taskonomy2018}. 

We use as a baseline the single-task models for each of the 11 tasks.

Overall, our evaluation covered 935 models and we provide in the supplementary material the detailed experimental setup of each setting.

%\subsection{Settings}
%In the following, we run our experiments under 11 different settings presented in table \ref{experimental-settings}, for a total of 699 models evaluated. 
%The different settings will allow us to evaluate the impact on multi-task robustness following different design choices:

%\begin{enumerate}
%    \item Using S2 and S3: We evaluate how layers sharing impacts the robustness of the network. 
%    \item Using S2, S7 and S10: We propose an improved version of the multi-task adversarial attack proposed in [] and we show that our improvement allow us to overcome the limitations of the previous approach.
%    \item Using S4, S7, S8 and S9: We evaluate how the model size impacts the robustness of multi-task models. 
%    \item Using S1 and S7: We evaluate how the perturbation size affects the robustness of individual tasks.
%    %\item Using S7: We evaluate the tasks similarity, and the impact of tasks combination to improve the multi-task model robustness
%    \item Using S11 and S12: We evaluate how the training epochs impact the robustness of the tasks.
%    %\item Using S7 and S10: 
%\end{enumerate}


\input{LaTeX/-metrics}

==> LaTeX/_hypothesis.tex <==
\subsection{Hypothesis evaluation}

\paragraph{First order approximation of the adversarial vulnerability}

We analyze in Fig~\ref{fig:vuln} the first order expansion hypothesis for a model with 3 tasks (s,d,D) where all the tasks are attacked.
\begin{figure}
     \centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/hypothesis/vuln_first_order.png}
         \caption{Link between the Adversarial vulnerability and its first order approximation (the expectation of the norm of the sum of the gradients).}
         \label{fig:vuln-firstorder}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/hypothesis/steps_first_order.png}
         \caption{Link between the number of steps of the attack and the norm of the gradient}
         \label{fig:vuln-steps}
     \end{subfigure}
        \caption{Adversarial vulnerability when attacking a model with 3 tasks (s,d,D)}
        \label{fig:vuln} 
\end{figure}

Fig~\ref{fig:vuln-firstorder} supports that the first order approximation is not a right approximation of the vulnerability of multi-task models. In particular, there is no linear correspondence between the two when the vulnerability increases. Fig~\ref{fig:vuln-steps} suggests that the relationship between the two changes when the number of attack steps increase. 

%Additional tasks combinations are detailed in supp. mat and also show that after some attack steps, the first order relationship does not hold.

\paragraph{Adversarial Vulnerability and number of tasks.}

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/hypothesis/adv_vuln.png}}
\caption{Adversarial vulnerability for different combination of tasks}
\label{vuln-nb-tasks}
\end{center}
\vskip -0.2in
\end{figure}

Figure~\ref{vuln-nb-tasks} shows the first order adversarial vulnerability for different combination of tasks (from 3 to 5 tasks). We show in the legend the successive addition of tasks to the model. As our theorem 7 showed, adding more tasks does not change monotonically the vulnerability of the model. The vulnerability keeps decreasing for combination (2), while it keeps increasing for combination (4), and combination (1) and (3) show a non monotonic relationship. It also shows that it is only when adding the segmentation task to any combination of tasks that the vulnerability drastically increases, which confirms Theorem 7 insights about the relationship between the marginal vulnerability and robustness of the additional task, irrespective with the total number of tasks we attack. Finally, it shows that starting from a vulnerable task (semantic segmentation in combination 2), we can dampen the overall vulnerability of the model by adding robust tasks.   


\paragraph{Adversarial vulnerability against L-$\infty$ norm attacks and L-$2$ norm attacks.}

We evaluate in this context the impact of using norm L2 in our attacks, under low perturbation amount (epsilon=4), and limited attack steps (25).
This configuration is the one demonstrated in Theorem 3 where multi-task learning makes it harder to attack individual and multiple tasks. While improving the robustness against L2 attacks, multi-task learning provides little defense against L-infinite attacks. 

Figure~\ref{fig:impact-norm} shows that the relative task robustness introduced by an L2 attack is very limited in comparison with what we can achieve with an L-infinite under the same configuration. Additional figures about the other tasks are in Appendix C.


\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{Figures/norm/relative_s.png}}
\vskip -0.2in
\caption{Impact of attack norm on the relative task robustness of image segmentation. Lower is better.}
\label{fig:impact-norm}
\end{center}
\vskip -0.4in
\end{figure}


\paragraph{Multi-task learning VS single-task learning.} If adding more tasks does not necessary yields better robustness, do multi-task models at least outperform single-task models?   


%\begin{figure}[]
%\begin{center}
%\centerline{\includegraphics[width=0.6\columnwidth]{Figures/monoVSmulti/result_resnet18_noW_mono_vanilla_relative.png}}
%\vskip -0.15in
%\caption{Relative task robustness when attacking the main task (row) with a model trained with an auxiliary task (column). Higher values mean more Error after attack, i.e less robust model.}
%\label{fig:resnet18_noW_mono_vanilla}
%\end{center}
%\vskip -0.3in
%\end{figure}

Under single-task attacks (Table ~\ref{table:tasks-opt} (A)), the multi-task model is more robust than the single-task model in only 40\% of the combinations. Under multi-task attacks, this ratio jumps to 60\%. This confirms that in general multi-task learning does not increase the robustness of models against single-task or multi-task attacks.



==> LaTeX/_study_factors.tex <==
\subsection{Other factors of adversarial robustness in multi-task learning}

We investigate in this section the other design choices that impact the robustness of multi-task models.

\paragraph{Task weight optimizations.}

The previous results have been obtained using the vanilla PGD attack proposed in \cite{yang2020multitask} on models where all the tasks had the same weights. Table \ref{table:tasks-opt} shows the relative task robustness of models under our two optimized attacks MGD (in B) and AGD (in C) to be compared with the baseline PGD (in A). In bold, the combination where the multi-task model is more robust than the single task model and in underline the combination of tasks where the Vanilla is stronger than our attacks.  

Our optimization MGD beats the Vanilla in 92\% of the tasks combinations in mono-task attacks and 60\% of the tasks combination in multi-task attacks, while MAGD beats the Vanilla attack in 86\% of the single-task attacks combinations and 55\% of the multi-task attacks while being 30\% cheaper to run than the baseline.

It is worth mentioning that single-task attacks causes more error than the multi-task error in 100\% of the combinations. Which confirms that even when the attack is optimized, it is easier focus the attack on one task than attack multiple tasks together.

Table \ref{table:tasks-opt}(D) presents the relative task robustness of the vanilla attack against models where the tasks have been weighted following the dataset's paper recommendations \cite{taskonomy2018}. In all combinations, the tuned models are more robust than the equally weighted models, which suggest than its the task tuning not the number of tasks that impacts the robustness of the models. 

\begin{table*}
\vskip -0.1in
%\vskip 0.15in
%\hskip 0.2in
\begin{center}
\begin{small}
\scalebox{0.77}{
\begin{tabular}{cc|ccccc|ccccc|ccccc|ccccc|}
\hline
Attack &  & \multicolumn{5}{c|}{Vanilla (A)} & \multicolumn{5}{c|}{MGD (B)} & \multicolumn{5}{c|}{AGD (C)} & \multicolumn{5}{c|}{Weighted (D)}\\
\hline
     & & s & d & D & n & E & s & d & D & n & E& s & d & D & n & E & s & d & D & n & E  \\
\hline
\multirow{5}{*}{Single} &s & \textit{0.82} & 0.86 & 0.97 & 0.96 & 0.93 & \textit{0.82} & \underline{0.86} & 0.97 & 0.97 & 0.94 & \underline{\textit{0.81}} &   \underline{0.84} &   \underline{0.96} &   \underline{0.96} &   \underline{0.93} & 0.47 &  0.52 &  0.57 &  0.58 &  0.54\\
& d & 5.74 & \textit{5.61} & \textbf{5.28} & 6.88 & 6.41 & 7.34 & \textit{5.63} & 7.09 & 9.86 & 9.63 & \textbf{7.72} &   \textit{7.87} &   \textbf{7.45} &  10.67 &  10.55 & 1.25 &  1.56 &  2.00 &  1.65 &  1.92\\
& D & \textbf{5.93} & \textbf{6.14} & \textit{6.4} & 7.12 & 8.31 & 7.59 & 8.53 & \textit{6.42} & 10.16 & 11.35 & \textbf{7.78} &   8.92 &   \textit{8.45} &  10.94 &  11.75 & 2.16 &  1.88 &  1.98 &  2.11 &  1.78\\
& n & \textbf{7.43} & \textbf{9.48} & \textbf{8.93} & \textit{10.82} & \textbf{9.08} & \textbf{9.1} & \textbf{12.64} & \textbf{11.29} & \textit{14.16} & \textbf{12.35} & \textbf{9.43} &  \textbf{13.49} &  \textbf{11.61} &  \textit{15.02} &  \textbf{13.40} & 6.61 &  9.46 &  8.09 &  8.62 &  8.14\\
& E & \textbf{12.93} & \textbf{19.29} & \textbf{18.44} & \textbf{15.16} & \textit{22.57} & \textbf{12.95} & \textbf{19.32} & \textbf{18.45} & \textbf{15.17} & \underline{\textit{22.38}} & \textbf{16.30} &  \textbf{26.70} &  \textbf{25.49} &  \textbf{26.64} &  \textit{31.29} & 6.44 &  5.50 &  8.02 &  5.49 &  7.70\\
\hline
  \multirow{5}{*}{Multi} &s & - & 0.85 & 0.96 & 0.95 & 0.91 & - & \underline{0.81} & \underline{0.92} & \underline{0.94} & \underline{0.9} & - & \textbf{\underline{0.64}} &   \underline{0.86} &   \underline{0.84} &   \underline{0.82}  & 0.47 &  0.45 &  0.49 &  0.48 &  0.43\\
& d & \textbf{1.99} & - & \textbf{5.42} & \textbf{4.8} & \textbf{4.46} & \textbf{4.63} & - & \textbf{5.44} & 7.66 & 6.71 & \textbf{2.69} &   - &   \textbf{7.36} &   \textbf{6.12} &   \textbf{4.78} & 0.56 &  - &  2.06 &  0.82 &  0.75\\
& D & \textbf{2.14} & \textbf{6.02} & - & \textbf{5.02} & 6.07 & 2.46 & 0.03 & - & 2.55 & 2.68 & \textbf{2.37} &   8.56 &   - &   \textbf{6.32} &   \textbf{\underline{5.98}} & 0.88 &  1.74 &  - &  0.94 &  0.68\\
& n & \textbf{4.61} & \textbf{9.4} & \textbf{8.93} & - & \textbf{8.7} & \textbf{5.68} & \underline{\textbf{6.07}} & \underline{\textbf{6.09}} & - & \underline{8.16} & \textbf{5.29} &   \textbf{\underline{8.65}} &   \textbf{\underline{7.58}} &  - &   \textbf{9.31} & 3.65 &  9.22 &  7.99 &  - &  6.32\\
& E & \textbf{7.58} & \textbf{18.5} & \textbf{17.44} & \textbf{12.48} & - & \textbf{10.04} & \underline{\textbf{12.39}} & \underline{\textbf{11.61}} & \textbf{13.61} & - & 6.70 &  \underline{10.37} &  \underline{10.69} &  \underline{12.12} &  - & 3.24 &  4.93 &  7.00 &  3.36 &  -\\
\hline
\end{tabular}
}
\vskip -0.1in
\caption{Relative Task Robustness under different settings}
\label{table:tasks-opt}
\end{small}
\end{center}
\vskip -0.3in
\end{table*}

\paragraph{Insights from figures in Appendix C.} Appendix C presents more figures on this section’s experiments. They yield additional insights which we summarize here.

\emph{Impact of the attack budget $\epsilon$.} Under strong adversarial attacks, auxiliary tasks do not provide reliable robustness both against single-task and multi-task adversarial attacks.

\emph{Impact of the model's architecture.} Madry et al.\cite{madry2017towards} has showed that smaller models are the most vulnerable against adversarial examples on MNIST[] and CIFAR[] datasets. Our results suggest that at the contrary, attacks on larger models cause more error under the same budget.

\emph{Training steps.} In multi-task learning, adding more training epochs improves both the clean performance and the robustness against single-task and multi-task attacks

==> LaTeX/_study_tasks.tex <==
\subsection{Study of the tasks}

In order to evaluate the relationships between tasks, we cannot immediately use the error or the loss values of the combinations as they have different scales and reflects different properties. Hence, we rely on the relative robustness metric we previously proposed and we use an ordinal approach to rank the interactions between the main task and each auxiliary as we assume that the task performance change monotonically. Starting from a matrix of relative task robustness (like Table~\ref{table:tasks-opt} A), we build a matrix of pairwise tournament between the auxiliary tasks. For each row $k$ of main task, the column $i$ of the auxiliary task indicates the number of other auxiliary combinations where the auxiliary task $i$ provides the best performances against. 

We compare different settings and run the following statistical tests in table~\ref{tbl:stats-atks}: \textbf{Pearson Correlation} on the relative task robustness metric and \textbf{Kendall Tau ranking} on the ordinal rankings of auxiliary tasks.

Our evaluation shows that auxiliary tasks that are comparatively better than others in mono-task attacks are also better in multi-task attacks (1) and that robust combination of tasks in mono-task attacks are also robust combinations in multi-task attacks (2).

The link between robustness and task transfer is statistically negligible (3 and 4), on the contrary of the link between robustness and learning. This confirms statistically that combinations of tasks that achieve higher clean performances are also the most robust both against mono-tasks and multi-task attacks (5 and 6).

Next, we show that the combination of tasks that are robust in one architecture are also robust in another architecture (8), and there is a strong evidence (p-value = 0.002, effect size $>$ 0.5) that auxiliary tasks that support a main task in one architecture also support this main task on an other architecture (7).

Similarly, we show that combination of tasks that are robust together with limited training remain the most robust when enough training budget (11 and 12).

Finally, we compared whether the overall robustness of the tasks combinations is similar between a Renet50 and a Resnet18 model, and according to the Wicoxon Two-sided, we cannot reject the null hypothesis at a confidence level of 5\% that the two architectures provide similar performances. However, if we test the hypothesis that the robustness in a Resnet50 model is higher than the robustness in a smaller model, the Wilcoxon-test shows that this hypothesis can be rejected at a confidence level of 5\%. This confirms that having larger models does not statistically improve the robustness of a multi-task model.

\begin{mdframed}[style=MyFrame]
We cannot infer the choice of the optimal combinations of tasks from their task transfer similarity, however evaluating their clean performances, evaluating their robustness in smaller models or after few training steps can hint which combination of tasks are more robust.
\end{mdframed}
%\textbf{We cannot infer the choice of the optimal combinations of tasks from their task transfer similarity, however evaluating their clean performances, evaluating their robustness in smaller models or after few training steps can also hint about which combination of tasks are preferable.}

\begin{table}[]
\begin{center}
\begin{small}
\scalebox{0.7}{
\begin{tabular}{c|c|c|cc}
\hline
  Metric1 & Metric2 & Test & effect size & p-value  \\
\hline
  \multirow{2}{*}{ST  Robustness} &  \multirow{2}{*}{Multi-task Robustness} & Kendall (1) &  0.724  & 9.798 e-06\\
  \cline{3-5}
   &  &  Pearson (2) & 0.93 & 8.41 e-12\\
\hline
   \multirow{2}{*}{MT Robustness} &  \multirow{2}{*}{Task Transfer(3)} & Kendall &  0.121  & 0.449\\
  \cline{3-5}
   &  &  Pearson & 0.20 & 0.33\\
\hline
   \multirow{2}{*}{ST Robustness} &  \multirow{2}{*}{Task Transfer (4)} & Kendall &  0.114  & 0.586\\
  \cline{3-5}
   &  &  Pearson & 0.08 & 0.70\\
\hline
   \multirow{2}{*}{MT Robustness} &  \multirow{2}{*}{Task Learning (5)} & Kendall &  -0.236 & 0.149\\
  \cline{3-5}
   &  &  Pearson & 0.94 & 2.58e-12\\
\hline
   \multirow{2}{*}{ST Robustness} &  \multirow{2}{*}{Task Learning (6)} & Kendall &  -0.156 & 0.341\\
  \cline{3-5}
   &  &  Pearson & 0.98 & 1.91e-17\\
\hline
   \multirow{2}{*}{Resnet50} &  \multirow{2}{*}{Resnet18} & Kendall  (7) & 0.51 & 0.002\\
  \cline{3-5}
   &  &  Pearson (8) & 0.94 & 1.42e-12\\
   \cline{3-5}
   &  &  Two-sided Wilcoxon (9) & 59 & 0.086\\
   
   \cline{3-5}
   &  &  Greater Wilcoxon (10) & 151 & 0.043\\
   \hline
   \multirow{2}{*}{50 epochs} &  \multirow{2}{*}{150 epochs} & Kendall (11) &  0.5 & 2.26e-3\\
  \cline{3-5}
   &  &  Pearson (12) & 0.55 & 4.23e-3\\
\hline
\end{tabular}
}

\end{small}
\end{center}
\caption{Statistical correlation between the different metrics. MT: Multi-task; ST: Single-Task}
\label{tbl:stats-atks}
\vskip -0.2in
\end{table}




%Knowing the robustness on two tasks (two by two), can we infer the robustness of 3 tasks? 

%The fact there is no correlation between transfer and robustness confirms that adding an auxillary task that is related to the main task according to Taxonomy (like D and d) does not make the model less or more robust.


%\paragraph{Collaborative tasks robustness}


%\subsection{Mono Robustness \& Multi-robustness}

%KendalltauResult(correlation=0.7240000000000001, pvalue=9.798288078869026e-06) 
%Pearson(0.8400000000000001, 1.5061643470464924e-07)

%\subsection{Robustness \& Transfer affinity}

%\paragraph{multi-task attacks:}
%Pearson Correlation between task robustness \& transfer affinity: (0.04063728734751635, 0.8470660239914007)
%Kendall Order correlation: KendalltauResult(correlation=0.12112702310050734, pvalue=0.44881922452403433)


%\paragraph{Mono-task attacks:}
%Pearson Correlation between task robustness \& transfer affinity: (0.11441169155894705, 0.5860528793676638)
%Kendall Order correlation: KendalltauResult(correlation=0.11721969977468451, pvalue=0.463586942852103)

%\subsection{Robustness on eps4 VS eps 8 VS eps16}

%\subsection{Robustness on epochs 5 VS 25 VS 50}

%\subsection{Noise per task}
%PSNR mean per task


%\subsection{Robustness \& Learning affinity}

%\subsection{Robustness \& Adversarial transferability}

==> LaTeX/_theoretical.tex <==
\subsection{Adversarial Vulnerability of multi-task models}

Simon et al. \cite{simon2019first} first introduced the concept of deep learning models vulnerability and linked it to the average gradient norm. \cite{yang2020multitask} applied the same definition and approximation to multi-task models. We extend the adversarial vulnerability to the second order and show later empirically that there is no one-to-one relationship between the average norms of the gradients and adversarial vulnerability in multi-task models and hence, the need to go beyond the first order approximation.  

In this section, we provide a theoretical evaluation of the adversarial vulnerability of multi-task models. The proofs are provided in the supplementary materials.

\paragraph{Definition 1.} Let $\mathscr{M}$  be a multi-task model with $\mathscr{T}= \{t_1,...,t_M\}$ tasks, an input $x$, $\bar{y} = (y_1, ..., y_M)$ its corresponding ground-truth.
We denote the set of attacked tasks $\mathscr{T}'$, a subset of the model's tasks $\mathscr{T}$. and the joint task loss of attacked tasks $\mathcal{L}'$. Then, we define the \emph{adversarial vulnerability} of $\mathscr{M}$ on $\mathscr{T}' \subseteq \mathscr{T}$ to an $\epsilon$-sized $\| .\|_p$-attack, the average increase-after attack over the whole dataset of the joint loss of the attacked tasks, i.e.:

%\scalebox{0.8}{
\begin{equation*}
    \left.\mathbb{E}_{x}[\delta \mathcal{L}'(x, \bar{y}, \epsilon, \mathscr{T}')]=\mathbb{E}_{x}\left[\max _{\|\delta\|_{p}<\epsilon} \mid \mathcal{L}'(x+\delta, \bar{y})-\mathcal{L}'(x, \bar{y})\right \mid \right]
\end{equation*}
%}

This definition matches the intuition of previous work \cite{goodfellow2015explaining, sinha2017certifying} about the robustness of deep learning models. The models are vulnerable when, on average over x, a small perturbation causes a large variation of loss.

Given the variation $\delta$ is small, we propose the following Taylor expansion in $\epsilon$:

\paragraph{Lemma 2.} Under an $\epsilon$-sized adversarial attack generated with a $\| .\|_p$ norm, the adversarial vulnerability of a multi-task model under a multi-task attack is
%\scalebox{0.7}{
\begin{equation}
\begin{aligned}
    \mathbb{E}_{x}[\delta \mathcal{L}'(x, \bar{y}, \epsilon, \mathscr{T}')]\approx \epsilon \cdot \mathbb{E}_{x}[\left\mid\mid \partial_{x} \mathcal{L}'(x, \bar{y}) \mid \mid_q\right] + \\ \frac{\epsilon^2}{2} \cdot \mathbb{E}_{x}[\left\mid\mid \partial^2_{x} \mathcal{L}'(x, \bar{y}) \mid \mid_q\right]
\end{aligned}
\label{lemme2}
\end{equation}

%}

where $q$ is the dual norm of $p$ and $\frac{1}{p}+\frac{1}{q}=1$ and $1 \leq p \leq \infty$.

We go beyond the first order expansion because our empirical results show in section XXX that the first order expansion is not sufficient. In particular: (1) when restricting the attack on the $l-\infty$ norm, the perturbation of the loss computed with the dual norm is non negligible. (2) When increasing the number of steps, under sufficient $\epsilon$, the high orders terms dominate of the expansion dominate. (3) The input noise is only adjusted with regards to the gradient of $\mathcal{L}'$ of the attacked tasks and increasing the number of jointly attacked tasks makes the noise harder to align with $\partial_{x} \mathcal{L}'$.  

Under this first order expansion, \cite{yang2020multitask} proposed the following theorem:

\paragraph{Theorem 3.} Consider a multi-task model $\mathscr{M}$ where an attacker attacks M tasks uniformly weighted with an $\epsilon$-sized adversarial attack under a $\| .\|_p$ norm. If the model is converged, and the gradient for each task is i.i.d. with zero mean and the tasks are correlated, a first order adversarial vulnerability of the model can be approximated as

\begin{equation}
\begin{aligned}
    \mathbb{E}_{x}[\delta \mathcal{L}']\approx K \cdot \sqrt{\frac{1+\frac{2}{M} \sum_{i=1}^{M} \sum_{j=1}^{i-1} \frac{\operatorname{Cov}\left(\mathbf{r}_{i}, \mathbf{r}_{j}\right)}{\operatorname{Cov}\left(\mathbf{r}_{i}, \mathbf{r}_{i}\right)}}{M}}
\end{aligned}
\label{theorem3}
\end{equation}

where K is a constant dependant of $\epsilon$ and the attacked tasks and $\mathbf{r}_{i}=\partial_{x} \mathcal{L}(x, y_i)$ the gradient of the task i and $\operatorname{Cov}\left(\mathbf{r}_{i}, \mathbf{r}_{j}\right)$ the covariance between the two gradients $\mathbf{r}_{i}, \mathbf{r}_{j}$.  

This theorem indicates that under a specific setting, (1) increasing the number of tasks reduces the adversarial vulnerability of models and (2) adding tasks with a low covariance of their gradients reduces the adversarial vulnerability as well.

In practice, this setting is hard to achieve. In section XX we show that removing one of the hypothesis cancels the apparent robustness of multi-task models.

To get a grasp of the impact of tasks on the multi-task vulnerability, we propose two complementary theorems that require less hypothesis and constrained setting. 


\paragraph{Lemma 4.} For a given multi-task model $\mathscr{M}$, let $\mathbf{r}_{i}=\partial_{x} \mathcal{L}(x, y_i)$ the gradient of the task i, with a weight $w_i$ such as the joint gradient of $\mathscr{M}$ is defined as $\partial_{x} \mathcal{L}(x, \bar{y}) = \sum_{i=1}^{M} w_i \mathbf{r}_{i}$. Let $\| .\|_q$ be a norm and $p$ an integer. We have:

\begin{equation}
\begin{aligned}
    \mathbb{E}_{x}[\mid\mid \sum_{i=1}^{M} w_i \mathbf{r}_{i} \mid \mid_q^{p}] \leq M^p \sum_{i=1}^{M} w_i^p \mathbb{E}_{x} \left[\mid \mid \left \mathbf{r}_{i} \right\mid \mid_q^{p} \right]
\end{aligned}
\label{lemme4}
\end{equation}

This lemma provides an upper-bound of the average norm of the gradients that we use to evaluate the upper bounds of the adversarial vulnerability in the following theorems.  

\paragraph{Theorem 5.} For a given multi-task model $\mathscr{M}$, let $\mathbf{r}_{i}=\partial_{x} \mathcal{L}(x, y_i)$ the gradient of the task i, with a weight $w_i$ and zero mean such as the joint gradient of $\mathscr{M}$ is defined as $\partial_{x} \mathcal{L}(x, \bar{y}) = \sum_{i=1}^{M} w_i \mathbf{r}_{i}$. The joint gradient averaged over x is bounded as follow: 

%\sqrt{ \left( \frac{dx}{hx} \right)^{\!\!2} +  \left( \frac{dy}{hy} \right)^{\!\!2} +  \left( \frac{dz}{hz} \right)^{\!\!2}}

\begin{equation}
\begin{aligned}
    \mathbb{E}_{x}[\mid\mid \partial_{x} \mathcal{L}(x, \bar{y}) \mid \mid_q] \leq \sqrt{ \sum_{i=1}^{M} \frac{M-1}{M} \sigma_i^2 - \frac{\sum_{i=1}^{M} \operatorname{Cov}\left(\mathbf{r}_{i}, \mathbf{r}_{j}\right)}{M} }
\end{aligned}
\label{theorem5}
\end{equation}

where $\sigma_i^2$ is the variance of the gradient of the task.

This theorem proposes an upper bound of the first term of adversarial vulnerability presented in  \ref{lemme2} and can also be applied to the second order Taylor expansion of the Lemma 2.

When $M\to\infty$, the second term that holds the interactions between the tasks drops to 0, and the adversarial vulnerability is then bounded by $M . \max _{i < M} \{\sigma_i \} $. Thin indicates that when we increase the number of tasks, it is the individual vulnerability of the tasks we add that matters rather than the interaction of tasks. 


While this theorem provides insights about what happens when the number of tasks is very large, it does not bound the vulnerability when a single task is added to the attacked model. To that purpose, we propose the concept of marginal adversarial vulnerability.


\paragraph{Definition 6.} Let $\mathscr{M}$  be a multi-task model with $\mathscr{T}_{M}= \{t_1,...,t_M\}$ tasks, an input $x$, $\bar{y} = (y_1, ..., y_M)$ its corresponding ground-truth.
We denote the set of attacked tasks $\mathscr{T}_{N}$ and $\mathscr{T}_{N+1}$, two subsets of the model's tasks $\mathscr{T}$ such as $\mathscr{T}_{N+1} = \mathscr{T}_{N} \cup {t_{N+1}}$ and $N+1 \leq M$, and let $\mathcal{L}'$ be the joint task loss of attacked tasks.

We call \emph{marginal adversarial vulnerability} of the model to an $\mathscr{T}',\epsilon$-sized $\| .\|_p$-attack the difference between the adversarial vulnerability over the task set $\mathscr{T}_{N+1}$ and the adversarial vulnerability over the task set $\mathscr{T}_{N}$ . 

\begin{equation*}
    \left.\Delta_{N} \mathbb{E}_{x}[\delta \mathcal{L}'] = \mathbb{E}_{x}[\delta \mathcal{L}'(x, \bar{y}, \epsilon, \mathscr{T}_{N+1})] - \mathbb{E}_{x}[\delta \mathcal{L}'(x, \bar{y}, \epsilon, \mathscr{T}_{N})] \right]
\end{equation*}



\paragraph{Theorem 7.} For a given multi-task model $\mathscr{M}$, let $\mathbf{r}_{i}=\partial_{x} \mathcal{L}(x, y_i)$ the gradient of the task i, with a weight $w_i$ and zero mean such as the joint gradient of $\mathscr{M}$ is defined as $\partial_{x} \mathcal{L}(x, \bar{y}) = \sum_{i=1}^{M} w_i \mathbf{r}_{i}$. The first order marginal vulnerability is bounded as follow: 


\begin{equation}
\begin{aligned}
    \Delta_{N} \mathbb{E}_{x}[\delta \mathcal{L}'] \leq \epsilon \cdot ((N+1) \cdot w_{N+1}\mathbb{E}_{x}[\mid \mid \mathbf{r}_{N+1} \mid \mid] +  \\
    N \cdot \max _{i<N+1} w_{i}\mathbb{E}_{x} [\mid \mid \mathbf{r}_{i} \mid \mid] )
\end{aligned}
\label{theorem7}
\end{equation}


When all the tasks have the same weight, $w_i = \frac{1}{N}$ and $w_{N+1} = \frac{1}{N+1}$ and we have:

\begin{equation*}
\Delta_{N} \mathbb{E}_{x}[\delta \mathcal{L}'] \leq \epsilon \cdot (\mathbb{E}_{x}[\mid \mid \mathbf{r}_{N+1} \mid \mid] + \max _{i<N+1} \mathbb{E}_{x} [\mid \mid \mathbf{r}_{i} \mid \mid] )
\end{equation*}

This theorem shows that the increase in the adversarial robustness when we add more tasks does not depend on the number of tasks already attacked but relates to how robust is the new task we are adding.

Both theorems \ref{theorem5} and \ref{theorem7} suggest that we should care more about the auxilliary tasks we are adding to the multi-task model than the number of tasks we target.


%\subsection{Theoretical Analysis}

%\paragraph{Second-order adversarial vulnerability}

%Simon-Gabriel et al.\cite{simon2019first} linked the norm of the gradients with the first order vulnerability of the model. \cite{yang2020multitask} showed that this first order vulnerability remains in multi-task models when dealing with L2-normed attacks. We provide a generalization of their work and hint that the first order approximation do not held with multi-step multi-task attacks with different norms.



%Definition of Main task

%Definition of Auxillary task

==> LaTeX/draft.tex <==
% RQ1

\subsection{First order approximation of the adversarial vulnerability}

The first hypothesis of Theorem 3 is that the adversarial vulnerability of models against a $\| .\|_p$ normed attack can be approximated as the average over the inputs of the norm $q$ of the gradient of the tasks, where q is the conjugate of p. Under multiple combinations of tasks and attack budget (number of iterations for an $l_\infty$ PGD attack) we check the linear relationship between the vulnerability and the gradient.

Our findings show that if under a limited number of steps, the first order is a good enough approximation, there is no linear relation between vulnerability and gradients under strong attacks, which hints that the adversarial expansion in lemma 2 may be dominated by higher-order terms under stronger attacks. 

%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/hypothesis/vuln_first_order.png}
%         \caption{Link between the Adversarial vulnerability $\mathbb{E}_{x}[\delta \mathcal{L}']$ and its first order approximation
%         $\mathbb{E}_{x}[\mid\mid \partial_{x} \mathcal{L}'(x, \bar{y}) \mid \mid_1]$ for two attack budgets
%         %(the expectation of the norm of the sum of the gradients).
%         }
%         \label{fig:vuln-firstorder}
%     \end{subfigure}
%     
%     \begin{subfigure}[b]{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/hypothesis/steps_first_order.png}
%         \caption{First-order approximation vs attack steps for $\epsilon=8$}
%        \label{fig:vuln-steps}
%     \end{subfigure}
%\vskip -0.1in
%     \caption{Adversarial vulnerability when attacking a model with 3 tasks (s,d,D)}
%    \label{fig:vuln} 
%     \vskip -0.1in
%\end{figure}


\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/hypothesis/vuln_first_order_eps8.png}}
\vskip -0.1in
\caption{Link between the Adversarial vulnerability $\mathbb{E}_{x}[\delta \mathcal{L}']$ and its first order approximation.
         %$\mathbb{E}_{x}[\mid\mid \partial_{x} \mathcal{L}'(x, \bar{y}) \mid \mid_1]$.
         %(the expectation of the norm of the sum of the gradients).
         }
\label{fig:vuln}
\end{center}
\vskip -0.3in
\end{figure}

In Fig~\ref{fig:vuln}, we evaluate the first-order expansion hypothesis for a model with 3 tasks (s, d, D) where all the tasks are attacked.
Fig~\ref{fig:vuln} supports that the first-order approximation is not a right approximation of the vulnerability of multi-task models, 
%under two different attack budgets $\epsilon=8$ and $\epsilon=2$. 
under an attack budget $\epsilon=8/255$.
In particular, there is no linear correspondence when the vulnerability increases, i.e. when we increase the strength of the attack.%number of iterations of the attack.

%Fig~\ref{fig:vuln-steps} suggests that the first order approximation when the number of attack steps increases and becomes exponential. 
Appendix C shows more task combinations where the first-order approximation of the vulnerability does not hold.
%Other task combinations also suggest that a higher-order approximation of the vulnerability is needed. 


\begin{figure}[]

\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/wgdVapgd2.png}}

\caption{Relative Task vulnerability between the single task model and the multitask combination against AutoPGD and WGD both when one task is attacked and when both tasks are attacked. Positive values mean that The Multitask combination is more robust than the single task.}
\label{fig:vuln-wgdpgd-tasks}
\end{center}

\end{figure}

==> LaTeX/old/_attacks.tex <==
\section{From single-task to multi-task attacks}

\subsection{Preliminaries}

Let $\mathscr{M}_{M}$ a multi-task model with $M$ tasks. For each input example, $x$ we denote by $\bar{y}$ the corresponding ground-truth label. 
In a multitask context, for each $x$, $y_i$ is the corresponding ground truth for task $i$ and we have $\bar{y} = (y_1, ..., y_M)$.

In our research, we focus on hard sharing multi-task learning, where the models are made of one encoder (backbone network common to all tasks) $E(.)$ and task specific decoders $D_i(.)$. Each task is associated with its corresponding loss $\mathscr{L}_i$ .

$$ \mathscr{L}_i(x,y_{i}) = l_i(D_i(E(x)),y_i)$$

where $l_i$ is a loss function tailored to the task $i$. For instance, we can use cross-entropy losses for classification tasks, while using L1 losses for regression tasks.

The total loss $\mathscr{L}$ of our multi-task model is a weighted sum of the individual losses $\mathscr{L}_i$ of each task:
$$ \mathscr{L}(x,\bar{y}) = \sum_{i=1}^{M} w_i \mathscr{L}_i(x, y_i)$$
where $\{w_1 \dots w_M\}$ are the weights of the tasks, either set manually or optimized during training \cite{}.

\paragraph{Single task adversarial attacks}

In this use case, the adversary tries to increase the error of one single task. This threat model can represent scenarios where the attacker has access to one task only or aims to perturb one identified task.  
The objective of the attacker in this case can be modelled as:

\begin{equation}
\underset{\delta}{\operatorname{argmax}} \: \mathscr{L_i}(x+\delta,y_i) \: \text{s.t.} \: \norm{\delta}{p} \leq \epsilon
\label{eq:single-task-objective}
\end{equation}
where $i$ is the index of the targeted class. 

One of the earliest proposed attacks is the Fast Gradient Sign Method (FGSM) \cite{Goodfellow14}. It adds a small perturbation \(\eta\) to the input of a neural network, which is defined as
\begin{equation}
\eta = \epsilon \, \text{sign}(\nabla_x \mathscr{L}_i(\theta,x,y_i)),\label{eq:fgsm}
\end{equation}
where \(\theta\) are the parameters of the network, \(x\) are the input data, \(y_i\) are the targets and \(\mathscr{L_i}(\theta,x,y_i)\) is the loss function used. Note that the required gradient is easily computed through backpropagation if the network structure is known (white-box).
%FGSM is a single step attack. 
Following Goodfellow, other attacks were proposed, first by adding iterations (I-FGSM\cite{}), projections and random restart (PGD\cite{}), momentum (MIM~\cite{}). All these attacks can be applied on a multi-task model when focusing on a single task. 

\paragraph{Multi task adversarial attacks}

In multi-task adversarial attacks, the adversary tries to increase the error of multiple outputs all at once. This captures scenarios where the adversary does not have a fine-grained access to the individual tasks or where the final prediction of the system results from the combination of multiple tasks (e.g., a self-driving car predicting steering angle by combining image segmentation and depth prediction \cite{}). Therefore, the adversary has to attack all tasks together. 

Given a multi-task model $\mathscr{M}$, $x$ an input example, and $\bar{y}$ the corresponding ground-truth label, 
the attacker tries to find the perturbation $\delta$ that will maximize the joint loss function of the attacked tasks  
the objective of a multi-task attack within a p-norm bounded distance $\epsilon$ is as follows:

\begin{equation}
 \underset{\delta}{\operatorname{argmax}} \: \mathscr{L}(x+\delta,\bar{y}) \: \text{s.t.} \: \norm{\delta}{p} \leq \epsilon 
\label{eq:multi-task-objective}
\end{equation}

While the interactions between different tasks are negligible when a single task is targeted (as shown in section XXX), attacking multiple tasks together brings the interactions between tasks into play and, thereby, affects the success rate of the attack.

Yang et al.\cite{yang2020multitask} have proposed a theoretical and empirical evaluation that hints that multi-task learning increases the robustness of models, however the demonstration and the empirical evaluation relied on multiple hypothesis that are hard to achieve in practice. It requires an $L2$ attack, with a valid first order approximation of the gradient, a converged model and a gradient of each task i.i.d with zero mean.

%\begin{enumerate}
%    \item The dual norm of the first order expansion of the weighted loss $\mathscr{L}$ is a sufficiently good approximation for the vulnerability of multi-task models to multi-task adversarial attacks
%    \item The gradient of each task is i.i.d. with zero mean when the models are converged.
%    \item The proof focused on the vulnerability of multi-task models to $L2$ attacksattacks.
%\end{enumerate}
%, raises the following questions: (1) How does weighting the loss as the training and and the attack affect 

We extend their analyse and first provide a formal generalization of the adversarial vulnerability of multi-task models, then empirically evaluate the hypotheses that lead to the apparent robustness of multi-task learning and finally propose an optimized attack where multi-task models are less robust than their single-task counterparts, and hence show the false sense of robustness provided by multi-task learning. Finally, we propose a framework to help practitioners choose which task can be learnt together to improve the robustness of models.


\input{LaTeX/-theoretical}

\input{LaTeX/-wpgd}

%Under an $\epsilon$-sized adversarial attack generated with a $\| .\|_p$ norm, the adversarial vulnerability of a multi-task model under a multi-task attack is

%Intuitively, a robust model should have smaller change of the loss given any perturbation of the input.

%\emph{Alternating weighted adversarial attacks}

%
%\subsection{Definitions and Preliminaries}
%\paragraph{Multi-task learning objectives}

%In the following, we denote $\mathscr{M}_{M}$ a multi-task model with $M$ tasks trained on a dataset $\mathscr{D}_t=\{(x^{(k)}, y^{(k)})\}^{N_{train}}_{k=1}$ and tested on a clean dataset $\mathscr{D}_c=\{(x^{(k)}, y^{(k)})\}^{N_{test}}_{k=1}$
%Let $x$ the input example, and $\bar{y}$ the corresponding ground-truth label.  $(x,\bar{y}) \in \mathscr{D_c}$

%We define a test set $\mathscr{D}={(x_k, \bar{y}_k)}^{N}_{k=1}$

%In a multitask context, $\bar{y} = (y_1, ..., y_M)$ and the total loss $\mathscr{L}$ of the model is a weighted sum of the individual losses $L$ of each task:

%$$ \mathscr{L}(x,\bar{y}) = \sum_{i=1}^{M} w_i L(x, y_i)$$

%In our research, we focus on hard sharing multi-task learning, where the models are made of one common Encoder (backbone network) $E(.)$ and a task specific decoder $D_i(.)$. Each task is associated with its corresponding loss function $l_i$ 

%$$ \mathscr{L}(x,\bar{y}) = \sum_{i=1}^{M} w_i l_i(D_i(E(x)),y_i)$$

%\paragraph{Multi-task adversarial attacks } %on a Multi-task model}

%In this use case, the adversary tries to increase the error of multiple outputs all at once. It represent the case where the adversary does not have a fine-grained access to the individual tasks, or when multiple tasks are then combined by the system for a final prediction and need therefore to be attacked together. For instance, a self-driving car may predict the steering angle from both an image segmentation task and a depth prediction task.  

%Given a multi-task model $\mathscr{M}$, $x$ an input example, and $\bar{y}$ the corresponding ground-truth label, 
%the attacker tries to find the perturbation $\delta$ that will maximize the joint loss function of the attacked tasks  
%the objective of a multi-task attack within a p-norm bounded distance $\epsilon$ is as follows:

%$$ \underset{\delta}{\operatorname{argmax}} \: \mathscr{L}(x+\delta,\bar{y}) \: \text{s.t.} \: \norm{\delta}{p} \leq \epsilon $$

%\paragraph{Single-task adversarial attacks on a Multi-task model}

%Similarily, we can only target the task i and restrict the multi-objective optimization to the sole task i:

%$$ \underset{\delta}{\operatorname{argmax}} \: \mathscr{L_i}(x+\delta,y_i) \text{s.t.} \norm{\delta}{p} \leq \epsilon $$


%\input{LaTeX/-theoretical}

==> LaTeX/old/_classification.tex <==
\section{Classification tasks}

To complement our study on dense tasks, we evaluate our weighted PGD attack on a two-tasks classifirs under the two variants M1 and M2.

Our results confirm that on M1 our weighted attack performs as well as attacking a single-task model (figures \ref{success1M1}, which confirms that multi-task learning, even when combining task that are semantically different (gender and ethnicity) provides little robustness improvement over a single-task model, even under small perturbations.

The experiments on the model M2 show that when the encoder output capacity is too small, increasing the perturbation size yields a lower success rate, which indicates that the adversarial examples lie in harder locations to find.     

\textbf{Conclusions: Multi-task models provides limited defense for classification tasks and the encoder capacity impacts the success rate of the attacks under large pertubrations}

\begin{figure}[t]

\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/model1_success0.png}}
\caption{Success rate of the 4 attack strategies on Task1 for model M1.}
\label{success1M1}
\end{center}

\end{figure}

\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/model1_success1.png}}
\caption{Success rate of the 4 attack strategies on Task2 for model M1.}
\label{success2M1}
\end{center}
\vskip -0.2in
\end{figure}


==> LaTeX/old/_study_architectures.tex <==
\subsection{Impacts of the Network}

%\paragraph{Layer sharing}


\paragraph{Task weighing}

We compare the robustness of models trained with task weighing against models that did not use any training optimization.

Figure \ref{fig:resnet18_W_mono_diff} tackles the mono-task attacks and shows that models that have weighted tasks are more robust in 56\% of the combinations (14/25). In the context of multitask models, figure \ref{fig:resnet18_W_multi_diff} shows a similar behaviour with 60\% of the tasks combinations are more robust when the tasks are weighted (15/25). In both cases, task D is the one that benefits more from weighing the different tasks while task n is more robust when the tasks are not weighted in 70\% of its combinations.

\textbf{Conclusion: While task weighing is a common multi-task learning practice to improve the performance of multitask models, it also improves the robustness of multi-task models in ~60\% of the cases.}


\begin{figure}
     \centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/weight/result_resnet18_mono_diff_relative.png}
         \caption{Mono-task attack}
         \label{fig:resnet18_W_mono_diff}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/weight/result_resnet18_multi_diff_relative.png}
         \caption{Multi-task attack}
         \label{fig:resnet18_W_multi_diff}
     \end{subfigure}
        \caption{Attacking both on the main (a) and auxiliary tasks (b) in multi-task models. The values are difference between relative robustness of the weighted models and the non-weighted model. Lines: Main tasks being evaluated, columns: auxiliary tasks not attacked. Negative values means more Error for the non weighted model, i.e weighted model is a more robust model.}
        \label{fig:resnet18_W}
\end{figure}



\paragraph{Network architectures}

We compare three architectures, Resnet18, Resnet50 and Xception in figure \ref{fig:impact-archs}. Madry et al.\cite{madry2017towards} has showed that smaller models are the most vulnerable against adversarial examples on MNIST[] and CIFAR[] datasets. Our results suggest that at the contrary, attacks on larger models achieve higher relative errors under the same budgets. 

\begin{figure*}
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/archs/arch_s.png}
         \caption{mIoU of Semantic segmentation task}
         \label{fig:s_arch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/archs/arch_D_.png}
         \caption{MSE of Euclidian Depth task}
         \label{fig:d_arch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/archs/arch_E.png}
         \caption{MSE of Edge occlusion task}
         \label{fig:D_arch}
     \end{subfigure}
      \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/archs/arch_d.png}
         \caption{MSE of Z-Depth task}
         \label{fig:E_arch}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/archs/arch_n.png}
         \caption{MSE of Normal}
         \label{fig:n_arch}
     \end{subfigure}
    \caption{Impact of the architecture choice on the performance of different tasks (relative robustness) \emph{Can be put as table to gain space}}
    \label{fig:impact-archs}
\end{figure*}

\paragraph{Training steps}

Figure\ref{fig:epochs_s} compares the impact of additional training epochs on both clean and adversarial performances for the semantic segmentation task (Other tasks are provided in supplementary material and show similar results). These results hint that contrary to single task learning, there is no apparent trade off between clean performances and adversarial performance when additional training is provided, both for multi-task attacks and single task attacks.

\emph{*** Check with more than 150 epochs?***}

\textbf{Conclusion: In multi-task learning, adding more training epochs improves the clean performance and the robustness against mono-task and multi-task attacks}

\begin{figure}[t]
\begin{center}
   \begin{subfigure}[b]{0.9\linewidth}
         \includegraphics[width=\linewidth]{Figures/epochs/clean_error_s.png}
         \caption{Error with clean inputs}
         \label{fig:epoch_s_clean}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.9\linewidth}
         \includegraphics[width=\linewidth]{Figures/epochs/adv_error_s.png}
         \caption{Error with adversarial inputs}
         \label{fig:epoch_s_adv}
     \end{subfigure}
\end{center}
   \caption{Impact of the training epochs on the performance of the multi-task model models with clean and adversarial inputs on semantic segmentation task. }
\label{fig:epochs_s}
\end{figure}

%\paragraph{Adversarial training}

==> LaTeX/old/_study_attacks.tex <==
\subsection{Impacts of the Attacks}

\paragraph{Single-task Learning \& Multi-task Learning}

\begin{figure}
     \centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/monoVSmulti/result_resnet18_noW_mono_vanilla_relative.png}
         \caption{Mono-task attack}
         \label{fig:resnet18_noW_mono_vanilla}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/monoVSmulti/result_resnet18_noW_multi_vanilla_relative.png}
         \caption{Multi-task attack}
         \label{fig:resnet18_noW_multi_vanilla}
     \end{subfigure}
        \caption{The values are relative task robustness when attacking only the main task (a) or both tasks (b) in multi-task models. Lines: main tasks being evaluated, columns: auxiliary tasks not attacked. Higher values mean more Error after attack, i.e less robust model.}
        \label{fig:resnet18_noW_vanilla}
\end{figure}


For both mono-task attacks (Fig~\ref{fig:resnet18_noW_mono_vanilla}) and multi-task attacks (Fig~\ref{fig:resnet18_noW_multi_vanilla}), the multi-task model is more robust than the mono-task model for 40\% (respectively 60\%) of the cases. 
%(10/25 \& 15/25). 
This shows that it is indeed harder to attack many tasks than focus on one task, however, in both cases multi-task models do not reliably increase the robustness of the models. In more than half of the cases, the single task task models are more robust than their multi-task equivalent.

Besides, in 85\% %(17/20) 
of the cases, attacking multiple tasks is harder than attacking one task when dealing with multi-task models.

%When studying the full 11 x 11 tasks combination (cf supplementary materials), we can draw the same conclusions.

%\find{\textbf{RQ2 Answer:} Our approach allows to see drastic changes based on different exit strategies. The progressive strategy offers in our experiments a better outcome than a hard or a cyclic strategy.}

%\begin{tcolorbox}[colback=white]
     \textbf{Conclusion: Multi-task models are slightly better than single-task model when they are under multi-task attacks. They are however in general less robust when the attack focuses on one task.}  
%\end{tcolorbox}

\emph{*** Check with more than 2 classes?***}


\paragraph{Vanilla PGD vs Weighted PGD}

We compare the performance of our optimized PGD attack with the vanilla PGD proposed in \cite{yang2020multitask}. Our optimization beats the vanilla in 92\% of the tasks combinations in mono-task attacks and 60\% of the tasks combination in multi-task attacks.

The mono-task W-PGD attack also causes more error than the multi-task error in 100\% of the combinations. Which confirms that even when the attack is optimized, it is easier focus the attack on one task than attack multiple tasks together.

\begin{figure}
     \centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/attacks/result_resnet18_noW_mono_diff_relative.png}
         \caption{Mono-task attack}
         \label{fig:resnet18_noW_mono_vanilla}
     \end{subfigure}
     
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\linewidth]{Figures/attacks/result_resnet18_noW_multi_diff_relative.png}
         \caption{Multi-task attack}
         \label{fig:resnet18_noW_multi_vanilla}
     \end{subfigure}
        \caption{The values are the difference between relative task robustness between W-PGD attack and the vanilla PGD attack in multi-task models. Lines: main tasks being evaluated, columns: auxiliary tasks not attacked. Positive values mean more Error after attack for the W-PGD attack, i.e stronger attack than the original PGD.}
        \label{fig:resnet18_noW_vanilla}
\end{figure}


%Heatmaps comme précédents.
%Peut être heatmap de la difference entre Vanilla vs Weighted?
%Ou Boxplot de la difference pour chaque metrique mesurée?
%Ou statistical test that the two distributions are similar?


%\begin{tcolorbox}[colback=white]
    \textbf{Conclusion: Using a weighted attack, the multi-task models are not more robust neither less robust in comparison with their mono-task counterparts.}  
%\end{tcolorbox}

\paragraph{Impact of number of steps}

\begin{figure}
 \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/steps/mIoU Segment VS step.jpeg}
         \caption{mIoU of Semantic segmentation task}
         \label{fig:mioU_sem_steps}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/steps/MSE depth_euclidean VS step.jpeg}
         \caption{MSE of Euclidian Depth task}
         \label{fig:mse_euclidian_steps}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
        \includegraphics[width=\linewidth]{Figures/steps/MSE depth_zbuffer VS step.jpeg}
       \caption{MSE of Z-Depth task}
      \label{fig:mse_zdepth_steps}
     \end{subfigure}
 \begin{subfigure}[b]{0.45\textwidth}
 \centering
 \includegraphics[width=\linewidth]{Figures/steps/MSE edge_occlusion VS step.jpeg}
  \caption{MSE of Edge occlusion task}
   \label{fig:mse_edgeocc_steps}
\end{subfigure}
\caption{Impact of attack steps on the performance of different tasks .Legend: The first letters are the tasks the model has been trained on. The second letters are the tasks that are attacked}
    \label{fig:impact-steps-curve}
\end{figure}


%\begin{figure*}
 %    \begin{subfigure}[b]{0.4\textwidth}
  %       \includegraphics[width=\linewidth]{Figures/steps/steps_boxplot_s.png}
%         \caption{mIoU of Semantic segmentation task}
%         \label{fig:s_steps}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\linewidth]{Figures/steps/steps_boxplot_D_.png}
%         \caption{MSE of Euclidian Depth task}
%         \label{fig:d_steps}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\linewidth]{Figures/steps/steps_boxplot_E.png}
%         \caption{MSE of Edge occlusion task}
%         \label{fig:D_steps}
%     \end{subfigure}
      %\begin{subfigure}[b]{0.4\textwidth}
      %   \includegraphics[width=\linewidth]{Figures/steps/steps_boxplot_d.png}
      %   \caption{MSE of Z-Depth task}
      %   \label{fig:E_steps}
     %\end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\linewidth]{Figures/steps/steps_boxplot_n.png}
%         \caption{MSE of Normal}
%         \label{fig:n_steps}
 %    \end{subfigure}
 %   \caption{Impact of attack steps on the performance of different tasks.}
 %   \label{fig:impact-steps}
%\end{figure*}


% plots from robust-mtl-rq/Metrics co-tasks impacts

Figures in Fig~\ref{fig:impact-steps} show the impact of iteration steps on the robustness of the different tasks. The first finding is that while the multi-task models and the mono-task models display similar robustness on one-step and few step attacks, the differences across the models widens as we increase the number of steps (nd attack on a nd model causes a 75\% increase in the MSE of z-depth in comparison with a d attack on the same nd model (figure \ref{fig:mse_zdepth_steps}).

Especially, some combinations of tasks are more sensitive to the number of iterations. While Ds attack on a Ds model plateau after 15 epochs, D attack on the same Ds model keeps increasing significantly (TODO: slope or value) with the number of steps  (figure \ref{fig:mse_euclidian_steps}). Similarly, Es attack on an Es model plateau after 10 steps, while E attack on the same Es model keeps increasing (figure \ref{fig:mse_edgeocc_steps}).
In general, against the same multi-task model, multi-task attacks tend to plateau much earlier,  


Against mono-task attacks, Mono-task models are neither the more robust or the less across the different tasks. For instance training a model with the two tasks d and D makes the model 12\% more robust than mono-task D (figure \ref{fig:mse_euclidian_steps}, however training the model on the tasks n and D makes the model 48\% less robust than the mono-task model D.

Similar behaviour happens against multi-task attacks. While it is easier to attack a single task model (task D) than attacking 2 tasks together, other combination of tasks are easier to attack than attacking one single task (E and s together are easier to attack than s alone in figure~\ref{fig:mioU_sem_steps}).  

%\begin{tcolorbox}[colback=white]
    \textbf{Conclusion: In general, when given sufficient steps multi-task models perform as poorly as a mono-tasks models and multi-task attacks plateau earlier than their multi-task counterparts.}  
%\end{tcolorbox}

%\emph{TODO: maybe need some statistic evidences rather than figure analysis?}


\paragraph{Impact of Epsilon}


\begin{figure*}
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/epsilon/epsilon_s.png}
         \caption{mIoU of Semantic segmentation task}
         \label{fig:s_eps}
     \end{subfigure}
     \hfill
     %\begin{subfigure}[b]{0.4\textwidth}
     %    \includegraphics[width=\linewidth]{Figures/epsilon/epsilon_d.png}
     %    \caption{MSE of Euclidian Depth task}
     %    \label{fig:d_eps}
     %\end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/epsilon/epsilon_E.png}
         \caption{MSE of Edge occlusion task}
         \label{fig:D_eps}
     \end{subfigure}
      \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/epsilon/epsilon_d.png}
         \caption{MSE of Z-Depth task}
         \label{fig:E_eps}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/epsilon/epsilon_n.png}
         \caption{MSE of Normal}
         \label{fig:n_eps}
     \end{subfigure}
    \caption{Impact of attack strength on the performance of different tasks. Epsilon axis (x) is logarithmic}
    \label{fig:impact-eps}
\end{figure*}


We evaluate our different tasks combinations under different strength of attacks. We present the results of 4 tasks in figure \ref{fig:impact-eps}, for each of the main tasks (s,D,E,n), the boxplots reflects the relative error across various auxiliary tasks,both in the mono-task attack context and in the multi-task context. Our results show that strength of attacks impact differently the different tasks. While, the image segmentation task (s) and the Normal prediction (n) task display a linear error with the increased epsilon, the Edge (E) and Depth tasks (D) show an exponential vulnerability to the strength of the attack. This different behaviour reflects both in multi-task attacks and mono-task attacks. It is worth noticing that this different behaviour cannot be explained by the nature of metric used (task S uses mIOu error and cross entropy loss while task n uses MSE and L1 loss) nor the amplitude of error (n and E have closer range of values than E and D).    

Our results also hint that under highs attack budgets, mono-task attacks and the multi-task attacks achieve close performance, while the variance of robustness provided by the different auxiliary tasks widens.

\emph{Can we explain all these differences?}

\textbf{Conclusion: Under strong adversarial attacks, auxillary tasks do not provide reliable robustness both against mono-task and multi-task adversarial attacks.}

\paragraph{Impact of Norm}

We evaluate in this context the impact of using norm L2 in our attacks, under low perturbation amount (epsilon=4), and limited attack steps (25).
This configuration is the one evaluated theoretically and empirically by \cite{yang2020multitask} where they showed that multi-task learning makes it very difficult to attack invidual and multiple tasks. Figure~\ref{fig:impact-norm} shows that the relative error introduced by an L2 attack is very limited in comparison with what we can achieve with an L-infinite under the same configuration. 


\textbf{Conclusion: While improving the robustness against L2 attacks, multi-task learning provides little defense against L-infinite attacks.}

\begin{figure*}
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/norm/relative_s.png}
         \caption{mIoU of Semantic segmentation task}
         \label{fig:s_norm}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/norm/relative_D_.png}
         \caption{MSE of Euclidian Depth task}
         \label{fig:d_norm}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/norm/relative_E.png}
         \caption{MSE of Edge occlusion task}
         \label{fig:D_norm}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.4\textwidth}
         \includegraphics[width=\linewidth]{Figures/norm/relative_d.png}
         \caption{MSE of Z-Depth task}
         \label{fig:E_norm}
     \end{subfigure}
     \hfill
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\linewidth]{Figures/norm/relative_n.png}
%         \caption{MSE of Normal}
%         \label{fig:n_norm}
%     \end{subfigure}
    \caption{Impact of attack norm on the performance of different tasks \emph{Can be put as table to gain space}}
    \label{fig:impact-norm}
\end{figure*}



\begin{table*}
%\vskip -0.1in
%\vskip 0.15in
%\hskip 0.2in
\begin{center}
\begin{small}
\hspace*{-.4cm}
\scalebox{0.76}{
\begin{tabular}{|cc|ccccc|ccccc|ccccc|ccccc|}
\hline
Attack &  & \multicolumn{5}{c|}{Baseline (A)} & \multicolumn{5}{c|}{MGD (B)} & \multicolumn{5}{c|}{AGD (C)} & \multicolumn{5}{c|}{Weighted (D)}\\
\hline
     \multicolumn{2}{|c|}{Auxiliary $\rightarrow$} & s & d & D & n & E & s & d & D & n & E& s & d & D & n & E & s & d & D & n & E  \\
\hline
\multirow{5}{*}{Single} &s & \textit{0.82} & 0.86 & 0.97 & 0.96 & 0.93 & \textit{0.82} & \underline{0.86} & 0.97 & 0.97 & 0.94 & \underline{\textit{0.81}} &   \underline{0.84} &   \underline{0.96} &   \underline{0.96} &   \underline{0.93} & 0.47 &  0.52 &  0.57 &  0.58 &  0.54\\
& d & 5.74 & \textit{5.61} & \textbf{5.28} & 6.88 & 6.41 & 7.34 & \textit{5.63} & 7.09 & 9.86 & 9.63 & \textbf{7.72} &   \textit{7.87} &   \textbf{7.45} &  10.67 &  10.55 & 1.25 &  1.56 &  2.00 &  1.65 &  1.92\\
& D & \textbf{5.93} & \textbf{6.14} & \textit{6.4} & 7.12 & 8.31 & 7.59 & 8.53 & \textit{6.42} & 10.16 & 11.35 & \textbf{7.78} &   8.92 &   \textit{8.45} &  10.94 &  11.75 & 2.16 &  1.88 &  1.98 &  2.11 &  1.78\\
& n & \textbf{7.43} & \textbf{9.48} & \textbf{8.93} & \textit{10.82} & \textbf{9.08} & \textbf{9.1} & \textbf{12.64} & \textbf{11.29} & \textit{14.16} & \textbf{12.35} & \textbf{9.43} &  \textbf{13.49} &  \textbf{11.61} &  \textit{15.02} &  \textbf{13.40} & 6.61 &  9.46 &  8.09 &  8.62 &  8.14\\
& E & \textbf{12.93} & \textbf{19.29} & \textbf{18.44} & \textbf{15.16} & \textit{22.57} & \textbf{12.95} & \textbf{19.32} & \textbf{18.45} & \textbf{15.17} & \underline{\textit{22.38}} & \textbf{16.30} &  \textbf{26.70} &  \textbf{25.49} &  \textbf{26.64} &  \textit{31.29} & 6.44 &  5.50 &  8.02 &  5.49 &  7.70\\
\hline
\hline
  \multirow{5}{*}{Multi} &s & - & 0.85 & 0.96 & 0.95 & 0.91 & - & \underline{0.81} & \underline{0.92} & \underline{0.94} & \underline{0.9} & - & \textbf{\underline{0.64}} &   \underline{0.86} &   \underline{0.84} &   \underline{0.82}  & - &  0.45 &  0.49 &  0.48 &  0.43\\
& d & \textbf{1.99} & - & \textbf{5.42} & \textbf{4.8} & \textbf{4.46} & \textbf{4.63} & - & \textbf{5.44} & 7.66 & 6.71 & \textbf{2.69} &   - &   \textbf{7.36} &   \textbf{6.12} &   \textbf{4.78} & 0.56 &  - &  2.06 &  0.82 &  0.75\\
& D & \textbf{2.14} & \textbf{6.02} & - & \textbf{5.02} & 6.07 & 2.46 & 0.03 & - & 2.55 & 2.68 & \textbf{2.37} &   8.56 &   - &   \textbf{6.32} &   \textbf{\underline{5.98}} & 0.88 &  1.74 &  - &  0.94 &  0.68\\
& n & \textbf{4.61} & \textbf{9.4} & \textbf{8.93} & - & \textbf{8.7} & \textbf{5.68} & \underline{\textbf{6.07}} & \underline{\textbf{6.09}} & - & \underline{8.16} & \textbf{5.29} &   \textbf{\underline{8.65}} &   \textbf{\underline{7.58}} &  - &   \textbf{9.31} & 3.65 &  9.22 &  7.99 &  - &  6.32\\
& E & \textbf{7.58} & \textbf{18.5} & \textbf{17.44} & \textbf{12.48} & - & \textbf{10.04} & \underline{\textbf{12.39}} & \underline{\textbf{11.61}} & \textbf{13.61} & - & 6.70 &  \underline{10.37} &  \underline{10.69} &  \underline{12.12} &  - & 3.24 &  4.93 &  7.00 &  3.36 &  -\\
\hline
\end{tabular}
}
\vskip -0.1in
\caption{Relative Task Robustness under 4 different settings: (A): the baseline PGD attack against uniformly weighted tasks. (B)\&(C): our MGD and AGD attacks. Each row refers to the main task evaluated and the column refers to the auxiliary task. In the top half (Single), we only attack the main task, in the bottom half (Multi), both tasks are attacked. 
In bold, the combinations where the multi-task model is more robust than the single-task model and in underline the combinations of tasks where the Baseline is stronger than our attacks.}
\label{table:tasks-opt}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}
